DeepER -- Deep Entity Resolution

Entity resolution (ER) is a key data integration problem. Despite the efforts in 70+ years in all aspects of ER, there is still a high demand for democratizing ER - humans are heavily involved in labeling data, performing feature engineering, tuning parameters, and defining blocking functions. With the recent advances in deep learning, in particular distributed representation of words (a.k.a. word embeddings), we present a novel ER system, called DeepER, that achieves good accuracy, high efficiency, as well as ease-of-use (i.e., much less human efforts). For accuracy, we use sophisticated composition methods, namely uni- and bi-directional recurrent neural networks (RNNs) with long short term memory (LSTM) hidden units, to convert each tuple to a distributed representation (i.e., a vector), which can in turn be used to effectively capture similarities between tuples. We consider both the case where pre-trained word embeddings are available as well the case where they are not; we present ways to learn and tune the distributed representations. For efficiency, we propose a locality sensitive hashing (LSH) based blocking approach that uses distributed representations of tuples; it takes all attributes of a tuple into consideration and produces much smaller blocks, compared with traditional methods that consider only a few attributes. For ease-of-use, DeepER requires much less human labeled data and does not need feature engineering, compared with traditional machine learning based approaches which require handcrafted features, and similarity functions along with their associated thresholds. We evaluate our algorithms on multiple datasets (including benchmarks, biomedical data, as well as multi-lingual data) and the extensive experimental results show that DeepER outperforms existing solutions.

==> advanced.tex <==
%!TEX root = main.tex
\section{Advanced Details [1 page]}
\label{sec:advanced}

\bi
	\item Other architectures
	\item Negative sampling 
	\item Adaptive learning
	\item Hyperparameter tuning
	\item Incorporating domain knowledge
	\item Handling other languages via fas text?
	\item Handling unknown domains via representation learning
\ei


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Revisiting Desiderata}
GiG


==> old_expt.tex <==
%!TEX root = main.tex
\section{Experimental Results}
\label{sec:expt}

We extensively evaluate our proposed approach along its different flavors and compare it to state-of-the-art ER methods on several real world datasets for which we have obtained the ground truth, \ie actual matching records.

\subsection{Experimental Setup}
\label{sec:setting}


\stitle{Datasets.}
Table~\ref{tbl:datasets} shows the datasets used in our evaluation. 
These datasets have been widely used to evaluate ER algorithms and systems.
In particular, we use three datasets from the bibliography domain, 
namely  \at{Pub_{DA}}={\bf DBLP-ACM}~\cite{benchmarks}, \at{Pub_{DS}}={\bf DBLP-Scholar}~\cite{benchmarks}, and \at{Pub_{DC}}={\bf DBLP-Citseer}~\cite{falcon}, 
and three datasets from the product domain, namely 
 \at{Prod_{AB}}={\bf Abt-Buy}~\cite{benchmarks}, \at{Prod_{AG}}={\bf Amazon-Google}~\cite{benchmarks}, and \at{Prod_{WA}}={\bf Walmart-Amazon}~\cite{GokhaleDDNRSZ14}, and finally one dataset from the restaurant domain, namely \at{Rest_{FZ}}={\bf Fodors-Zagats}~\cite{uis}.
For each of these datasets, we obtained the actual matching pairs. 
Many of these have been obtained manually by their authors.
In the table, we list the number of tuples in the first and second tables, the number of matching pairs, and the number of attributes in each table.
 
 
 \begin{table}[t!]
{\scriptsize
\begin{center}
\begin{tabular}{|c| c | c | c | }
\hline
~
   & {\bf Size (1st - 2nd)}
   & {\bf \#Matching Pairs} 
   & {\bf \#Attr} 
%   & {\bf Description}
\\ 	\hline
	\at{Pub_{DA}}  & \at{(2,616 - 2,294)} & \at{2,224} & \at{4} \\ %& \at{}\\
	\hline
	\at{Pub_{DS}} & \at{(2,616 - 64,263)} & \at{5,347} & \at{4} \\ %& \at{} \\
	\hline
	\at{Pub_{DC}} & \at{(1,823,978 - 2,512,927)} & \at{558,787} & \at{4} \\ %& \at{} \\
	\hline
	\at{Prod_{AB}} & \at{(1,081 - 1,092)} & \at{1,097} & \at{4} \\ %& \at{}\\
	\hline
	\at{Prod_{AG}} & \at{(1,363 - 3,226)} & \at{1,300} & \at{5} \\ %& \at{ } \\
	\hline
	\at{Prod_{WA}} & \at{(2,554 - 22,074)} & \at{1,154} & \at{17} \\ %& \at{} \\
	\hline
		\at{Rest_{FZ}} & \at{(533 - 331)} & \at{112} & \at{7} \\ %& \at{} \\
	\hline
	\multicolumn{4}{|c|}{
	\at{Pub_{DA}}={\bf DBLP-ACM}, \at{Pub_{DS}}={\bf DBLP-Scholar} }   \\
	\multicolumn{4}{|c|}{
	\at{Pub_{DC}}={\bf DBLP-Citseer} }   \\
	\multicolumn{4}{|c|}{
	\at{Prod_{AB}}={\bf Abt-Buy}, \at{Prod_{AG}}={\bf Amazon-Google} 
}\\
	\multicolumn{4}{|c|}{\at{Prod_{WA}}={\bf Walmart-Amazon},	\at{Rest_{FZ}}={\bf Fodors-Zagats}} \\
	\hline
\end{tabular}
\end{center}
} % end of font
%\vspace*{-3ex}
\caption{Dataset statistics} %\paolo{can we make it richer with number of attributes and any other feature (\% of nulls?)?}} \rohit{Have uniform representation 100K and 5K or exact numbers like 100567, 5345} \paolo{agree}
\label{tbl:datasets}
%\vspace*{-2.5ex}
\end{table}


%\stitle{Comparisons with Existing Approaches.}
%We evaluated our approach against 

\stitle{Hardware and Software Setup.}
All experiments were run on a machine with ...
We implemented \sys in XXX ...\mourad{Mohamed, please fill in}

\stitle{Parameters.} 
\mourad{Mohamed, please fill in}

\stitle{Parameters Performance Evaluation.}
\mourad{Mohamed, explain the different parameters, the number of runs and how they were done, etc. }

We report the average Precision, Recall, and F-measure obtained across ....


\subsection{Comparison with Existing Methods}


On the right side of Table~\ref{table:comparison}, we report the best F-measures values obtained from previously published works.
We mainly focus on the experimental study of different entity resolution approaches reported in~\cite{erhard2010, soru2014} and 
on two  state-of-the-art crowd-based systems, namely Corleone~\cite{corleone} and Falcon~\cite{falcon}.
The authors of~\cite{erhard2010} studied three non learning and two ML-based approaches under different parameters.
For the non-learning approaches, they use an undisclosed commercial system (COSY) and PPJoin+~\cite{}.
For the learning approaches, they sue SVM inside FEBRL~\cite{} and MARLIN~\cite{} which uses SVM and decision trees.
They use 500 training pairs where the ratio of match and non-match pairs is guided by a ratio method they have optimized.
The authors  of~\cite{soru2014} studied ten machine learning approaches; four  linear non-probabilistic classifiers, 
four rely on probability theory, one uses a multilayer perceptron, and one is rule-based (decision table).
Corleone is an crowd-based platform for ER that aims at removing the need of developers.
It uses the crowd to train a learning-based matcher.
Falcon is a follow-up work to scale Corleone using RDBMS-like query execution and optimization on top of Hadoop.
We added Falcon so we can have as it was the only system that was run on the \at{Pub_{DC}} dataset. 
The best F-measure values obtained by any of these methods is reported in the table.
While these numbers may not be directly comparable, they are the best that these different approaches and systems have achieved
after fine-tuning their different parameters.




%reports the precision, recall, and F-measure obtained by \sys using its light and heavy versions.
%These numbers were obtained by setting the training data size at XX\% with a ratio of match and non-match pairs of Y:Z.
%We run ...\mourad{Mohamed, fill in and explain}
%We also report the best F-measure obtained from previously published works.
%We mainly focus on the experimental study of different entity resolution approaches reported in~\cite{erhard2010} and 
%on two  state-of-the-art crowd-based systems, namely Corleone~\cite{corleone} and Falcon~\cite{falcon}.
%The authors of~\cite{erhard2010} studied two three non learning and two ML-based approaches under different parameters.
%The best F-measure values obtained by any of these methods is reported in the table and we differentiate between the learning and non-learning by the superscript (NL and L, respectively).
%Corleone is an crowd-based platform for ER that aims at removing the need of developers.
%It uses the crowd to train a learning-based matcher.
%Falcon is a follow-up work to scale Corleone using RDBMS-like query execution and optimization on top of Hadoop.
%We added Falcon so we can have as it was the only system that was run on the \at{Pub_{DC}} dataset. 
%While these numbers may not be directly comparable, they are the best that these different approaches and systems have achieved
%after fine-tuning their different parameters.

Looking at the different numbers in the table, we see that \sys delivers superior performance over all datasets even in its light version ...
\sys achieves small improvements on the X, Y, Z datasets which have been noted to be easy in the literature and for which the published works already achieve good results.
However, we see more pronounced improvement on the more difficult datasets, namely W, T, ......\mourad{We need to say more after we see the numbers!}



%\setlength{\tabcolsep}{3pt}
\begin{table*}[ht!]
\center
\small
\begin{threeparttable}
\begin{tabular}{|c|c|c|c||c|c|c||c|c|c|c|c|}
%\hline
\hline
 Dataset  
 & \multicolumn{3}{c||}{\sys Light}
 & \multicolumn{3}{c||}{\sys Heavy} 
 & \multicolumn{3}{c|}{Published Works(F)} 
%&Published Works (F)
\\
 %& $P$ & $R$ & $F$ &  $P$ & $R$ & $F$ & $P$ & $R$ & $F$ \\
 & $P$ & $R$ & $F$ &  $P$ & $R$ & $F$ &  $Rule$ &  $ML$  &  $Crowd$ \\ 
 \hline
   	\at{Pub_{DA}}	& & & & &	& & 97.6~\cite{erhard2010}\tnote{1} & 97.6~\cite{erhard2010}\tnote{2} - 97.81~\cite{soru2014}\tnote{3} &\\	
	\at{Pub_{DS}}  & & & & &	& & 84.5~\cite{erhard2010}\tnote{4}  & 89.4~\cite{erhard2010}\tnote{5} & 92.1~\cite{corleone}\\
	\at{Pub_{DC}} & & & & &	& & & & 95.2~\cite{falcon}\\
   	\at{Prod_{AB}}	& & & & &	& & 70.7~\cite{erhard2010}\tnote{4} & 71.3~\cite{erhard2010}\tnote{2}&\\	
	\at{Pub_{AG}}  & & & & &	& & 62.2~\cite{erhard2010}\tnote{4} &60.1~\cite{erhard2010}\tnote{2} &\\
	\at{Pub_{WA}} & & & & &	& & &&89.3~\cite{corleone}\\
	\at{Rest_{FZ}} & & & & &	& & &&96.5~\cite{corleone}\\
\hline
\end{tabular}
\begin{tablenotes}
    \item[1]FEBRL FellegitSunter.     $^2$FEBRL SVM.  $^3$ Linear SVM.     $^4$ COSY (Undisclosed commercial system).     $^5$ MARLIN SVM
  \end{tablenotes}
\end{threeparttable}
%\vspace{-2ex}
\caption{Comparing the performance of \sys in its two forms to published works. }
\label{table:comparison}
\end{table*}




\subsection{Varying the Size of the Training Data}

In this experiment, we show how \sys behaves when the training data is varied \wrt to the total numbers of perfect matching pairs.
In a typical scenario, we would like to limit the required training data as much as possible, as it is usually expensive to obtain.
\mourad{Can we say something about positive examples being harder/more expensive to obtain than negative examples and somehow argue that we still do not require a lot of labeling effort since we could use a 1:N ratio where N>1 and still get good results?}

Table~\ref{table:training} shows the results of our experiments. 
While as expected, we obtained better results at higher sizes of the training data, we are still having good performance even at a 10\%
ratio ...\mourad{We need to say more after we see the numbers!}

\begin{table*}%[ht!]
\center
\small
\begin{tabular}{|c|c|c|c||c|c|c||c|c|c||c|c|c|}
%\hline
\hline
 Dataset  
 & \multicolumn{3}{c||}{@10\%}
 & \multicolumn{3}{c||}{@25\%}
 & \multicolumn{3}{c||}{@50\%}
 & \multicolumn{3}{c|}{@80\%}
\\
 & $P$ & $R$ & $F$ 
 &  $P$ & $R$ & $F$  
 &  $P$  & $R$ & $F$ 
 &  $P$ & $R$ & $F$\\ 
 \hline
   	\at{Pub_{X?}}	 & & & & &	& &  & & & &	&   \\	
   	\at{Prod_{Y?}}	& & & & &	& & & & & &	& \\	
	\at{Rest_{FZ}} & & & & &	& &  & & & &	&\\
\hline
\end{tabular}
%\vspace{-2ex}
\caption{Varying the size of training data in \sys. }
\label{table:training}
\end{table*}


\subsection{The Effect of Noise in the Training Data}

We already mentioned that obtaining training data is expensive, worst it is not necessarily perfect.
In this experiment, we show the robustness of \sys when the training data is noisy, that is 
some of the labels for matching and non-matching pairs are incorrect.
Interestingly, to our advantage, most of the existing literature did not study this aspect well\mourad{Is it true!?}


Table~\ref{table:noise} shows the results of our experiments. ...\mourad{We need to say more after we see the numbers!}

\begin{table*}%[ht!]
\center
\small
\begin{tabular}{|c|c|c|c||c|c|c||c|c|c||c|c|c|}
%\hline
\hline
 Dataset  
 & \multicolumn{3}{c||}{@10\%}
 & \multicolumn{3}{c||}{@25\%}
 & \multicolumn{3}{c||}{@50\%}
 & \multicolumn{3}{c|}{@80\%}
\\
 & $P$ & $R$ & $F$ 
 &  $P$ & $R$ & $F$  
 &  $P$  & $R$ & $F$ 
 &  $P$ & $R$ & $F$\\ 
 \hline
   	\at{Pub_{X?}}	 & & & & &	& &  & & & &	&   \\	
   	\at{Prod_{Y?}}	& & & & &	& & & & & &	& \\	
	\at{Rest_{FZ}} & & & & &	& &  & & & &	&\\
\hline
\end{tabular}
%\vspace{-2ex}
\caption{Using training data @ 10\% while varying the noise. }
\label{table:noise}
\end{table*}

\subsection{Evaluating the robustness of \sys blocking}



==> overview.tex <==
%!TEX root = main.tex
\section{Background}
\label{sec:overview}

%One of the key contributions of our paper is an elegant synthesis of ideas from the theory of Entity Resolution (ER) and Deep  Learning (DL). In this section, we give an overview of the main techniques and how they all fit together.

Let $D = \{t_1, \ldots, t_n\}$ be a set of entities with $n$ tuples and $m$ attributes $\{A_1, \ldots, A_m\}$.
Note that these entities can come from one table or multiple tables (with aligned attributes).
We denote by $t_i[A_j]$ the value of attribute $A_j$ on tuple $t_i$.

\subsubsection*{Entity Resolution}

The problem of {\em entity resolution} (ER) is, given all distinct tuple pairs $(t_i, t_j)$ from $D$ where $t_i \neq t_j$, determine which pairs of tuples refer to the same real-world entities (\aka~a {\em match}).


\subsubsection*{Entity Resolution as a Classification Problem}

ER is typically treated as a binary classification problem~\cite{theoryrecordlinkage,DBLP:journals/tkde/ElmagarmidIV07,naumann2010introduction,DBLP:conf/kdd/BilenkoM03}.
%
%\stitle{Entity Resolution as a Classification Problem.}
%Most machine learning (ML) based approaches treat ER as a binary classification problem~\cite{theoryrecordlinkage,DBLP:journals/tkde/ElmagarmidIV07,naumann2010introduction,DBLP:conf/kdd/BilenkoM03}. 
Given a pair of tuples $(t_i, t_j)$, the classifier outputs \True~(resp. \False) to indicate that $t_i$ and $t_j$ match (resp. mismatch).
The Fellegi-Sunter model~\cite{theoryrecordlinkage} is a formal framework for probabilistic ER 
and most prior machine learning (ML) works are simple variants of this approach.

Intuitively, given two tuples $t_i$ and $t_j$, we compute a set of similarity scores between aligned attributes, based on predefined similarity functions. 
The vectors of known matched (resp. mismatched) tuple pairs -- that are also referred to as positive (resp. negative) examples -- 
are used to train a binary classifier (\eg SVMs,  decision trees, or random forests). 
The trained binary classifier can then be used to predict for any arbitrary tuple pair.

%\stitle{Distributed Representations (DRs) for Tuples.}
\subsubsection*{Word Embeddings for Unstructured Data}

Word embeddings map individual words to a dense high dimensional vector (say with 300 dimensions) such that semantically related concepts (such as ``Mac Phone" and ``iPhone") are close to each other in the vector space~\cite{mikolov2013distributed}.

Extensions of \wes such as Doc2Vec~\cite{} and Sentence2Vec have been proven effective over unstructured data.

\subsubsection*{Word Embeddings for Structured Data (Tuples)}

%A {\em distributed representation} of words (\aka\ {\em word embeddings})  maps individual words to a dense high dimensional vector (say with 300 dimensions) such that semantically related concepts (such as ``VLDB" and ``ICDE") are close to each other in the vector space~\cite{mikolov2013distributed}. \sys transforms each tuple into a high dimensional vector such that similar tuples have high similarity.

Apparently, we can compute the similarities of two entities in different granularities: attribute-level or tuple-level.
%

\etitle{Attribute2Vec.}
For attribute-level similarity, we need to convert each attribute value $v$ (a list of words) into its corresponding \DR, \eg by averaging the word vectors of each word $s$ in $v$ obtained from Glove~\cite{pennington2014glove}.

Naturally, the similarity between two attribute values can be computed as the distance between their corresponding vector representations, using \eg the cosine similarity. 

\etitle{Tuple2Vec.}
Alternatively, we can further compose the vector representations of each attribute of a tuple into a single vector representation, using sophisticated compositional methods such as long short term memory (LSTM) based recurrent neural networks (RNNs).


 

\add{==================}

%Our initial approach converts each attribute of the tuple into its corresponding distributed representation by averaging the word vectors obtained from Glove~\cite{pennington2014glove}.
%The similarity between two values for an attribute can be computed as the 
%distance between their corresponding vector representations, for example, using the cosine similarity metric.
The similarity vector is a $m$-dimensional vector where the $i$-th entry is the similarity score for attribute $A_i$ for the given pair of tuples.
A classifier is then trained based on the similarity vectors for known matched and mismatched tuple pairs.

%An alternate approach treats the entire tuple as a document
%and computes its DR as either the average of the DR of its attributes or through sophisticated DL techniques such as LSTM. 

An alternate approach computes a representation for each attribute through sophisticated compositional methods in DL such as LSTM-based recurrent neural networks. %treats the entire tuple as a document
%and computes its DR as either the average of the DR of its attributes or through sophisticated DL techniques such as LSTM. 
Given composed vectors for a pair of tuples, we compute their {\em distributional similarity} 
through subtracting (vector difference) or multiplying (Hadamard product) the corresponding entries.
The ER classifier is then trained based on the distributional similarity vector for the training examples.
%One can also use sophisticated compositional models, such as bi-directional recurrent neural network with long short-term memory  hidden units \cite{Hochreiter:1997}. 
%we outperform the state-of-the-art in all benchmark datasets.

%\stitle{Tuning Representations for Entity Resolution.}
%Almost all of the benchmark datasets for ER are in the English language and are general purpose domains such as matching products and publications. 
%Hence, we can use any of the popular pre-trained representations such as GloVe~\cite{pennington2014glove},
%word2vec~\cite{mikolov2013distributed}
%(or fastText~\cite{bojanowski2016enriching} for multilingual datasets).
%However, these representations are generic in the sense that they are not ``tuned'' for the specific ER task. 
%We propose an end-to-end mechanism to learn the appropriate representation for a particular dataset. 
%
%\stitle{Blocking for Distributed Representations.}
%Blocking is a key technique for improving the efficiency of ER by grouping tuples into blocks.
%There has been extensive work on designing appropriate blocking functions that operate in the symbolic realm.
%We propose two efficient and effective blocking algorithms based on the distributional representation for tuples 
%that also take semantic relatedness into account.
%
%\stitle{Overall Approach.}
%Algorithm~\ref{alg:metaER} shows the pseudocode for our overall approach.
%We describe how each of the steps is instantiated in the remainder of the paper.

\begin{algorithm}[t!]
     \caption{\sys Approach}
     \label{alg:metaER}
     \begin{algorithmic}[1]
        \STATE Convert each tuple into a compositional distributed representation
		\STATE Compute a similarity vector for each pair of tuples in the training set
		\STATE Train a classifier on the similarity vectors
		\STATE Perform blocking for all tuples in the dataset
		\STATE Run the classifier over all tuple pairs within each block
		\STATE Return all matched tuple pairs
     \end{algorithmic}
 \end{algorithm}

\add{==================}

%\red{If we have space, we should probably add a block diagram showing the same thing as Algorithm~1.}\mourad{Agree!}


==> response.tex <==
% !TEX root = main.tex


\twocolumn [\begin{center}\ttlfnt{PVLDB 2018 Paper 946: Author Response to Reviews of \\Distributed Representations of Tuples for Entity Resolution}\end{center}]

%\begin{center}
%\section*{Responses to Reviewers for:}
%\subsubsection*{Distributed Representations of Tuples for \\ Entity Resolution}
%\end{center}

%\vspace{1.8ex}
%\ni {\bf{\em Dear PVLDB Reviewers and Meta-Reviewer:}}
%\vspace{1.8ex}


\stab
We would like to thank the reviewers for their pertinent comments 
based on which we have made significant changes to improve the paper. 
%
We present below our responses to the reviewers and the meta-reviewer.
The major changes in the paper are highlighted in \add{blue}.

\subsection*{Summary of Major Changes.}
\begin{itemize}
    \itemsep-1mm
    \item We modified our paper to provide detailed justifications for our various design choices.
        These include and not limited to our choices for 
        (i)~distributed representations (\DRs), 
        (ii)~compositional approaches (AVG and LSTM-RNN), and 
        (iii)~how negative examples were constructed from positive examples.
    \item We  made a number of changes so that the paper is self-contained.
        These include additional discussions on how the LSH hash families for cosine similarity are constructed 
        and an intuitive description of how multi-probe LSH works.
    \item We conducted a number of new experiments such as evaluating Paragraph2Vec as a candidate for composition,
        and comparing different \DRs (GloVe vs. Word2Vec vs. FastText).
    \item We extended our experiments with additional datasets.
        For example, we now evaluate \sys against all of the 21 most heavily studied organisms in molecular biology.
        We also updated Figures~\ref{fig:varyingTrainingData}-\ref{fig:varyingComposition} with additional benchmark datasets.
        Furthermore, we added a large dataset for our multi-lingual experiment.
%    \item \red{Anything that I am missing?}
\end{itemize}

\input{rev1}
\input{rev2}
\input{rev3}

\setcounter{figure}{0}
\setcounter{table}{0}





==> response_shepherd.tex <==
% !TEX root = main.tex


\twocolumn [\begin{center}\ttlfnt{PVLDB 2018 Paper 1161: Author Response to Reviews of \\Distributed Representations of Tuples for Entity Resolution}\end{center}]


\stab
We would like to thank the reviewers for providing an additional chance to further improve our paper.
Below is a summary of the major changes we made, followed by our detailed responses to the reviewers and the meta-reviewer. 
For convenience,  changes introduced to this revision are in \add{blue}.


%\subsection* {Responses to the Meta-Reviews}

%The reviewers were underwhelmed by the revisions. The revisions were quite extensive and the authors resubmitted in only one month choosing to not address all the comments. 
%A revision decision is recommended. Here are the revisions:
%\begin{enumerate}
%\item  the authors should narrow the scope of the paper, such as, explicitly analyzing in which applications (e.g., where the word order is informative) the proposed techniques would really work.
%\item Include Table 1, which is now only in the response letter, in the paper.
%\item It would be good if the authors evaluate the blocking techniques by also considering the matcher, instead of an independent evaluation (as indicated in W1 of Reviewer 1).
%\item Please consider addressing the other issues raised including R1 W2, W3, D3, D5, or explicitly reduce the claims made in the paper to a narrower scope.
%\end{enumerate}

\subsection*{Summary of Major Changes.}

\begin{itemize}
    \itemsep-1mm
    \item We have conducted additional experiments to evaluate the end-to-end performance of both matching and blocking.
    \item We have updated our experiment on compositional approaches to include the Sentence2Vec performance from Table~1.
    \item We have clarified the potential limitations of our approach and the corresponding avenues for future work (summarized in the final remarks of the paper).
\end{itemize}


\input{rev1}
\input{rev2}
\input{rev3}

\setcounter{figure}{0}
\setcounter{table}{0}





==> rev1.tex <==
% !TEX root = main.tex

\subsection*{Responses to the Comments of Reviewer 1.}

\etitle{R1(W1).} 
{\em
For example, how does different LSH blocking options affect final linkage results? Will the extra pairs to compare cause more false positives (precision loss)? 
I didn't find new experiments added for this. The original experiments only show the performance of LSH independently, but not about its impact on downstream matching.}

\stab
{\bf [A]}  
%A discerning point!
%
Indeed, a bad blocking can cause loss in both precision and recall.
We measured the efficacy of blocking using two widely-used metrics, namely Reduction Ratio (RR) and Pair Completeness (PC).
PC is the ratio of the number of true duplicates compared by our approach against the total number of duplicates.
A \emph{lower} value of PC results in \emph{reduced recall} as some of the actual duplicates will not be in the same block and hence will not be compared.
RR is the ratio of the number of tuple pairs compared by our approach to the number of all possible pairs. 
A \emph{higher} value of RR implies a bad blocking where we will have to 
classify a lot of non-duplicates that could potentially result in \emph{reduced precision}.
Our prior experiment showed the impact of LSH on the PC and RR metrics in Figure~\ref{fig:blockingFigs}.

%\add{
Based on the reviewer's suggestion, we conducted a new experiment (new Figure~\ref{fig:blockingEndToEnd} in Page~\pageref{fig:blockingEndToEnd})
%}
where we studied the impact of LSH blocking on the precision and recall of \sys.
%\add{
For the reviewer's convenience, we have also included the new experiment in the response  (see Figure~\ref{fig:blockingEndToEndResp}).
%}
The results of these experiments are quite similar to those of Figure~\ref{fig:blockingFigs} in Page~\pageref{fig:blockingFigs}). 

Recall that for a fixed $L$, increasing $K$ resulted in decreased PC and RR (see Figures~\ref{fig:blockingFigs} a-b).
The corresponding impact on recall and precision can be found in Figures~\ref{fig:blockingEndToEnd} a-b.
The \emph{recall decreases} with increased $K$ as more and more duplicates are not put in the same block which results in \sys missing them.
The precision \emph{increases mildly} with increasing $K$ as an increasing number of spurious non-duplicates are no longer being compared.
For example, when $K=1$, almost half of all possible pairs are classified by \sys which reduces the precision with potential false positives.
However, when $K=10$, only a quarter of all possible pairs are classified, resulting in mild increase of precision.
The reason for the mild increase is that the classifier of \sys is relatively robust and achieves high precision even for low value of $K$.

For a fixed $K$, increasing $L$ resulted in an increase of both PC and RR (see Figures~\ref{fig:blockingFigs} c-d).
The corresponding impact on recall and precision can be found in Figures~\ref{fig:blockingEndToEnd} c-d.
As expected, the \emph{recall increases} with higher $L$ as almost all the true duplicates are put in the same block and end up being classified as such by \sys.
Since \sys is quite accurate, this results in an increased recall.
The precision \emph{declines mildly} with increasing $L$.
The reason is that more and more non-duplicates are put in the same block resulting in potential false positives.
Once again, the impact is mild as the classifier is relatively robust.

\begin{figure*}[t!p]
     \centering
     \mbox{
             \subfigure[K vs Recall (L=10)]{\includegraphics[width=125pt]{figures/blocking_vary_k_recall.pdf}}
             \subfigure[K vs Precision (L=10)]{\includegraphics[width=125pt]{figures/blocking_vary_k_precision.pdf}}
             \subfigure[L vs Recall (K=4)]{\includegraphics[width=125pt]{figures/blocking_vary_l_recall.pdf}}
             \subfigure[L vs Precision (K=4)]{\includegraphics[width=125pt]{figures/blocking_vary_l_precision.pdf}}
     }
  \vspace*{-3ex}         
     \caption{Impact of varying K and L on Precision and Recall of \sys }
     \label{fig:blockingEndToEndResp}
  \vspace*{-2ex}         
\end{figure*}


\etitle{R1(W2).} 
{\em
Paragragh2Vec
I'm not convinced that ``many attributes contain multi-word content'' infers ``considering the word order is important''. Bag of words can go quite far. I do like Table 1 in the author response, but am disappointed that the revision does not include the discussion or even mention Paragraph2Vec.
}


\stab
{\bf [A]} 
We indeed agree with the reviewer.
We reproduce below Table~\ref{tbl:varyingCompositionSentence2Vec} from the previous response for convenience.
Note that in all but one of the benchmark datasets (namely Prod-AG) that we evaluated, 
the AVG variant of \sys, which uses the bag of words approach,
performed comparably to the more sophisticated RNN-LSTM approach.
Hence, almost all of the experiments in our paper were conducted using the AVG approach.
The exceptions were Table~\ref{tbl:deepERBestPerf} (Page~\pageref{tbl:deepERBestPerf}) that shows that \sys could beat the state of the art (whether due to AVG or RNN-LSTM)
and Figure~\ref{fig:varyingComposition}  (Page~\pageref{fig:varyingComposition}) where we evaluated different composition methods. 


\begin{table}[h!]
\begin{tabular}{|c|c|c|c|c|}
    \hline
    {\bf Dataset} & {\bf AVG} & {\bf LSTM} & {\bf P2Vec} & {\bf Tuned P2Vec} \\ \hline
    Pub-DA &    98.63 &     98.44 &     90.12 &  96.12 \\ \hline
    Pub-DS &    97.04 &     95.45 &     88.47 &   92.74 \\ \hline
    Pub-DC &    96.82 &     99.6  &     90.29 &   91.33 \\ \hline
    Prod-AG &   77.53 &     91.44 &     73.25 &   80.54 \\ \hline
    Prod-WA &   86.3  &     89.06 &     81.3  &  83.2 \\ \hline
    Rest-FZ &   100   &     100   &     100   &  100 \\ \hline
\end{tabular}
%\vspace{-2ex}
 \tabcaption{Comparing Compositional Approaches}    
    \label{tbl:varyingCompositionSentence2Vec}
%\vspace{-4ex}
\end{table}

While AVG performs well, there are certain datasets,  such as Prod-AG,
% (duplicate products in Amazon-GoogleProducts), 
where RNN-LSTM has a role to play.
These datasets often have long product descriptions where a sophisticated approach seems to perform better.
%\add{
Understanding and automatically recommending the appropriate architecture for a given dataset is a key focus of our future research. 
We have updated our revised paper to qualify our claims that RNN-LSTM works best when word order is important. 
%}

We have added the content of Table~\ref{tbl:varyingCompositionSentence2Vec} to Figure~\ref{fig:varyingComposition} (Page~\pageref{fig:varyingComposition})
where we compare the performance of AVG, RNN-LSTM with a tuned version of Sentence2Vec.
Note that we used the term Sentence2Vec instead of Paragraph2Vec in the paper. 
%\add{to be consistent with the terminology proposed in~\cite{le2014distributed}.}
%\add{
Based on the reviewer's comment, we now include a larger discussion of Sentence2Vec in the description for Figure~\ref{fig:varyingComposition}.
%}





\etitle{R1(W3).} 
{\em
The review says even using 10\% training data the proposed method still perform similarly, whereas baseline such as random forest has much lower performance. I'm skeptical on this claim (and no data are shown) because it is well known that deep learning requires a lot of training data, comparing with other methods.}

\stab
{\bf [A]}
Our claim is based on two arguments: 
(a)~prior methods such as SVM and Random Forest perform poorly for small training data and 
(b)~\sys shows only mild decrease in performance even when only 10\% of training data is used.
Let us clarify both arguments.

\stitle{Impact of Training Data on SVM and Random Forest.}
A number of prior works have observed that traditional ML-based methods require 
a considerable amount of training data for ER. 
For a very recent discussion, please refer to Section 2.1 of~\cite{dong2018data} and the references therein.
We summarize the major observations.
Even for hand-tuned feature engineering, simple ML models such as SVM and Decision trees require as much as 500 training labels.
While this achieves $\sim$90\% F-measure on easy datasets, they only achieve $\sim$70\% F-measure on harder datasets.
Using more sophisticated models such as Random Forests requires double the number of training labels (almost 1000)
but achieves a F-measure of $\sim$95\% and $\sim$80\% on easy and hard datasets respectively.
The authors also note that to achieve F-measures of around 99\% with Random Forests (somewhat similar to \sys), 
one might require as much as 1.5 million training labels \emph{even for relatively clean datasets}.
Another recent work~\cite{anhaisigmod2018} observed that traditional methods such SVM or Random Forest 
quickly plateau and do not show increase in performance measure when training data increases (see Figure~6 in Appendix of~\cite{anhaisigmod2018}).

%\add{In a paper published in 2010, Rahm et al.\cite{FrameworksForEntityMatchingAComparison_dke2010} compared several ER methods including many that depend
%on training data. In their comparison (cf. Table 3), we clearly see that most methods require a large 
%number of training examples, not less than 50\% to achieve the best reported performance.\mourad{Need to double check}.
%In another paper~\cite{erhardvldb2010}, the ML methods that have been tested need 500 examples (with at least  at least 40\% being either
%matching or non-matching) to achieve good performance on the  datasets related to products,  which correspond to at least 20\% positive examples.
%In~\cite{psernan2017}, the evaluation is conducting using 80\% training data which is quite high.
%}\mourad{Not sure we can make a sweeping statement about the literature?}

We also conducted a new experiment (shown in Figure~\ref{fig:varyingTrainingDataDLRFSVM})
that compares the drop in performance of SVM, Random Forest, and \sys for reduced training data.
However, we do not include the complete table in the revised version of the paper due to the fact that this is well known and  the lack of space.
However, the behavior of \sys for varying training data size is included in Figure~\ref{fig:varyingTrainingData} (Page~\pageref{fig:varyingTrainingData}).

\begin{figure*}[!t]
   \centering
   \includegraphics[width=\textwidth]{figures/ResponseVaryingTrainingData.pdf}
%   \vspace*{-3ex}
   \caption{Impact of Training Data on Various Classifiers}
  % \vspace*{-3ex}
	\label{fig:varyingTrainingDataDLRFSVM}
\end{figure*}

\stitle{Impact of Training Data on \sys.}
Note that Figure~\ref{fig:varyingTrainingData} of our previous revision studied the impact of reduced training data on \sys.
The results show that impact is relatively minimal. 
It might seem that this flies in the face of conventional wisdom that says that DL models require a lot of training data.
However, \sys leverages two fundamental ideas in DL - transfer learning and appropriate DL architecture - to require less training data as explained below\footnote{For an additional discussion of how these factors help in reducing training data for data cleaning purposes, 
please refer to~\cite{thirumuruganathan2018data} and the references therein.}:

\begin{enumerate}
    \itemsep-1mm
    \item \emph{Transfer Learning:} 
        The fundamental idea behind transfer learning is to transfer - either the classifier or the (distributed) representation - from one dataset to another.
        In Computer Vision, there is a number of DL models trained on a large dataset such as ImageNet.
        If one wants to use DL for a small dataset, one can simply take the model trained on ImageNet 
		and ``tune'' it for a smaller dataset~\cite{yosinski2014transferable}.
        The intuition is that the larger DL model has learned some domain independent features when trained over ImageNet that can be reused for a related task on a smaller task.
%
        This is also the intuition behind using distributed representations (\DRs) for NLP tasks. 
        The \DRs are often trained on a very large corpus such as the Common Crawl or Wikipedia with billions of tokens.
        Learning a \DR~\cite{mikolov2013distributed} from these large datasets automatically imbues them with desired properties such as semantic similarity.
        \sys leverages this fact and uses the pre-trained \DRs to solve the ER problem.
        Due to the ``knowledge'' that has been transferred by using the \DRs, the amount of required training data  is comparatively smaller.

    \item \emph{Appropriate DL Architecture:}
        Another common technique to reduce training data is to choose a domain specific DL model.
        For example, both fully connected DL models, where each node is connected to every other node in the next layer,
        and convolutional neural networks (CNNs), where each node is only connected to other nodes that are spatially nearby,
        have similar expressive power for computer vision tasks.
        However, CNNs require dramatically less training data as the underlying architecture makes 
        additional assumptions (for example, spatial locality, hierarchy of representations, and so forth)~\cite{yosinski2014transferable} that reduce the amount of required training data.
%
        \sys also leverages this idea.
        Note that our proposed architecture in Figure~\ref{fig:ERmodel} is explicitly designed for entity resolution.
        It has two layers and does very simple mathematical operations.
        The compositional layer learns how to compose \DRs of words to \DRs of tuples while the
        similarity layer computes the similarity between \DRs of tuples.
        These are lightweight operations that can be learned very efficiently.
        Once the distributional similarity for tuples is computed, building a classifier does not require a lot of training data.
\end{enumerate}

\etitle{R1(D3).} 
{\em
Requiring manually ordering the attributes is a big drawback. Also, the paper does not discuss what if there are missing values (so the tuple would not be aligned). 
}

\stab
{\bf [A]} 
We would like to note that when using the AVG similarity, the ordering of attributes is not necessary.
For RNN-LSTM, an appropriate ordering can improve the performance. 
There is a number of heuristics to alleviate this. For example, one could mine functional dependencies and  use it for ordering, \eg
if \emph{Country} $\rightarrow$ \emph{Capital} is a functional dependency, one could order the attributes such that Country and Capital are nearby to each other. 

Currently, we replace missing values with \textsc{Unk},
%\add{
which are then retrofitted - see Section~\ref{subsec:substantialcover} or R1D5.
%}.

We have updated the paper to clarify these issues.

\etitle{R1(D5).} 
{\em
IDs provide important information for matching. Again I'm skeptical that simply treating all IDs as UNK can give better results.
}

\stab
{\bf [A]} 
Indeed IDs can potentially infuse additional information.
Our current \sys architecture relies primarily on \DRs that are trained on a large corpus such as 
the common crawl or Wikipedia.
It is likely that IDs are not present in these corpora and hence are replaced with 
the \textsc{Unk} representation which is then tuned by retrofitting.
%\add{
A key focus of our future work is to design a hybrid system that leverages both 
automatic features, such as \DRs, 
and manual features, such as a similarity metric for IDs.
%}

In the meanwhile, there are three potential ways to alleviate this issue. 
\begin{itemize}
    \itemsep-1mm
    \item \emph{Retrofitting.}
        Currently, \sys uses retrofitting to tweak \DRs obtained from GloVe to be more representative of the current dataset. 
        If words $W_i$ and $W_j$ occur a lot in a given dataset, they will have similar retrofitted \DRs even if they were far apart in GloVe.
        As mentioned in Section~\ref{subsec:substantialcover}, we replace each \textsc{Unk} with the average of $K$ of its most co-occurring words.
        For IDs, they are often words from the same tuple.
        So the \DRs of IDs will be very close to the average of their words from their corresponding tuples.
    \item \emph{Using Character based \DRs.}
        One could also use character based \DRs such as FastText.
        If a word such as \emph{ABCDE} is not present, then it looks up if some of its subwords are present in the DR.
        Such subwords could be \{A, AB, ABC, B, BC, BCD, $\ldots$\}. 
        Even if the entire ID is not present in the \DR dictionary, it is likely that some of its subwords are.
        FastText then simply averages all the \DRs of the subwords found in the dictionary.
        Combined with retrofitting, this can provide an excellent approximation.
    \item \emph{Learning \DRs for IDs automatically from the Data.}
        Ideally, if one has sufficient data, one can learn the \DRs from the data itself.
\end{itemize}


==> rev2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
% !TEX root = main.tex

\subsection*{Responses to the Comments of Reviewer 2.}

\etitle{Comment 1.} 
{\em
Include Table 1, which is now only in the response letter, into the revised version, if there is still enough space.
}

\stab
{\bf [A]} 
We have updated Figure~\ref{fig:varyingComposition} in Page~\pageref{fig:varyingComposition} with the contents of Table~1 from our response.
It now compares how various compositional techniques such as AVG, RNN-LSTM and Sentence2Vec perform for the benchmark datasets.

%\begin{table}
%\begin{tabular}{|c|c|c|c|c|}
%    \hline
%    {\bf Dataset} & {\bf AVG} & {\bf LSTM} & {\bf P2Vec} & {\bf Tuned P2Vec} \\ \hline
%    Pub-DA &    98.63 &     98.44 &     90.12 &  96.12 \\ \hline
%    Pub-DS &    97.04 &     95.45 &     88.47 &   92.74 \\ \hline
%    Pub-DC &    96.82 &     99.6  &     90.29 &   91.33 \\ \hline
%    Prod-AG &   77.53 &     91.44 &     73.25 &   80.54 \\ \hline
%    Prod-WA &   86.3  &     89.06 &     81.3  &  83.2 \\ \hline
%    Rest-FZ &   100   &     100   &     100   &  100 \\ \hline
%\end{tabular}
%\vspace{-2ex}
% \tabcaption{Comparing Compositional Approaches}    
%\vspace{-4ex}
%\label{tbl:compcompar}
%\end{table}


==> rev3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
% !TEX root = main.tex

\subsection*{Responses to the Comments of Reviewer 3.}

\etitle{Comment 1.} 
{\em
The authors used title and description as examples to argue the importance of word order, while such order-sensitive attributes are not always available in a dataset. Thus, I think such claim should be qualified in this paper. The authors also discussed connecting related attributes, but this is a technique to improve the performance of LSTM-RNN with a good initial state rather than the reason for choosing LSTM-RNN. The response letter did not address the case when word order is not preserved in a single attribute, e.g., ``Bill Clinton'' and ``Clinton, Bill'', or the case when dirty data (``Bill Clinton'' vs ``Bill Cliton'') or multiple representations (``25/06/2018'' vs ``Jun 25, 2018'') exist. 
}

\etitle{R3(W1).} 
{\em
RNN+LSTM is utilized to generate \DRs for tuples. The method lacks justification, though some good results are shown.
}

\stab
{\bf [A]}
We thank the reviewer for the insightful comments.
We completely agree with all of these observations.

\stitle{AVG vs. LSTM-RNN.}
As shown in Table~\ref{tbl:varyingCompositionSentence2Vec}, AVG, which is a compositional approach that ignores word ordering,
has a comparable performance with the more sophisticated LSTM-RNN based approach except in 
the Prod-AG dataset where it
seeks to identify duplicates in Amazon-Google Products, which have detailed descriptions.
Hence, for most datasets, AVG composition is quite sufficient.
The AVG composition can also handle some of the examples mentioned in the comment such as ``Bill Clinton'' and ``Clinton, Bill'' or 
``25/06/2018'' vs ``Jun 25, 2018'' (at least for the components 25 and 2018). 

However, for some of the more complex datasets such as Prod-AG, LSTM-RNN does have a role to play.
We would like to clarify that LSTM-RNN is not a silver bullet.
There are datasets where it might provide good performance while AVG might suffice for most datasets. 
LSTM-RNN also requires substantial computation time while AVG can be computed in a matter of seconds.
%\add{
Hence, understanding and automatically recommending the appropriate architecture for a given dataset is a key focus of our future research.
In other words, we must only use the expensive LSTM-RNN when the extra computational time produces a corresponding increase in F-measure performance.
We have updated our revised paper (Under ``{A Compositional Approach - RNN with LSTM}'' in Page~\pageref{subsec:lstm}) to qualify our claims that RNN-LSTM works best when word order is important.
%}

\stitle{Dirty Data.}
Our current architecture does not adequately handle dirty data corresponding to typos. 
The retrofitting approach proposed in Section~\ref{subsec:substantialcover} can potentially alleviate this issue
as the set of common words co-occurring with ``Clinton'' and ``Cliton'' might be quite similar.
Hence retrofitting could result in similar \DRs for both these words. 
An alternative approach would be to use character/sub-word level embeddings such as FastText
to  approximate the DR for ``Cliton'' as the average of multiple sub-words such as \{c, cl, cli, li, lit, it, ito, $\ldots$\}.

%\stitle{Action.}
%\add{
%}

